Formalising lexical and syntactic diversity for data sampling in French

Diversity is an important property of datasets and sampling data for diversity is useful in dataset creation. Finding the optimally diverse sample is expensive, we therefore present a heuristic significantly increasing diversity relative to random sampling. We also explore whether different kinds of diversity -- lexical and syntactic -- correlate, with the purpose of sampling for expensive syntactic diversity through inexpensive lexical diversity. We find that correlations fluctuate with different datasets and versions of diversity measures. This shows that an arbitrarily chosen measure may fall short of capturing diversity-related properties of datasets.

==> 1-intro-OLD.tex <==
%Why are we doing this ?
\todo{MOdify th eintroduction to highlight the importance of diversity and the lack of formalization in NLP }
Morphosyntactic treebanks are cornerstones of grammar induction \cite{zhu-etal-2020-return} and of 
morphosyntactic parsing, whether in monoligual \cite{dary-etal-2022-dependency}, multilingual \cite{straka-2018-udpipe} or cross-lingual \cite{glavas-vulic-2021-climbing} contexts. 
They help to probe language models for linguistic knowledge possibly encoded therein \cite{Shen-et-al-2023}, and for challenges, e.g. related to syntactic constructions, which they might fail to appropriately address \cite{bonial-tayyar-madabushi-2024-construction}. 

Treebanks are also fundamental resources in  research on language. They enable studying linguistic properties within or across languages \cite{Levshina-et-al-2023},
examining the appropriateness of language universals \cite{brosa-rodriguez-kahane-2024-new}, formalising and searching for complex phenomena such as constructions \cite{weissweiler-etal-2024-ucxn} or documenting low-resourced and endangered languages and dialects \cite{pugh-tyers-2024-universal}, inter alia. 

For many such research questions, manually annotated treebanks are not enough to check generalisations and touch upon long-tail phenomena \cite{sheinfux:wg2:book}. In such cases, corpora automatically annotated for morphology \cite{BARONI2009} and/or syntax \cite{vanNoord2013,ginter13ftb3} are used \cite{Schneider-2011-EN-varieties,bloem-etal-2014-applying}.

%Our objective is to build such a large, but still manageable, morphosyntactically parsed corpus for 
%French.\draftnote{marie:insister plus dès maintenant sur le focus de maximiser la diversité et pas la taille?}. 
%Reformulé: 
Our objective is to build such morphosyntactically parsed corpus for 
French which would fulfil two conditions. First, it should be large but manageable, i.e. its parsing, storage and maintenance cost should not be prohibitive. 
Second, it should still have  sufficient lexical and morphosyntactic diversity to serve studies in which long-tail phenomena play important roles, such as %word sense 
frame induction \cite{qasemizadeh-etal-2019-semeval}, %\draftnote{marie:cette ref concerne l'induction de frames. Enlever l'exemple du WSI?}
identification of multiword expressions (MWEs) unseen in manually annotated corpora \cite{ramisch-etal-2020-edition}, probing language models for rare but interesting syntactic phenomena \cite{misra2024languagemodelslearnrare,weissweiler2024hybridhumanllmcorpusconstruction}, etc. 

To this aim, %, crucial for long-tail phenomena, %we firstly attend to source text genres, like proposed in previous efforts \cite{przepiorkowski-etal-2010-recent,Davies-COCA-2010}. Secondly, we also we aim at selecting texts on the basis of formal lexical and morphosyntactic diversity. However, measuring morphosyntactic diversity requires pre-exiting morphosyntactic annotation
we use very large raw corpora including HPLT \cite{de2024new} and we rely on formal lexical and morphosyntactic diversity measures. We face, however, two tractability problems: (i) while lexical diversity can easily be calculated for a raw text, finding the optimally diverse subset of a very large set of texts is intractable, (ii) morphosyntactic diversity quantification requires the source data to be  parsed in advance, which is prohibitive in case of very large source corpora. 


%TODO: Objectives: corpus-induced semantic lexicon. Hypothesis: syntax approximates semantic roles. Jointly with distributional semantics, it should allow to induce a FrameNet-type lexicon whose granularity and accuracy matches a very corpus of French. 
%\todo{Cite papers on FrameNet induction shared task.}

%TODO: Extension of this application to MWE discovery, which remains a major challenge due to critical hardness from unseen data. The hypothesis is that outliers in the frame clustering process may correspond to MWE senses of predicates.

%Syntactically annotated corpora are important tools for studying and validating linguistic hypotheses.\todo{Cite a paper Nurit, and computational typology, e.g. Kahane et al., } 

In this context, %we hypothesise that lexical diversity can be efficiently combined with heuristic methods, and that it can be used as a proxy for morphosyntactic diversity. More precisely, 
we propose a data selection method, based on a heuristic, which is faster than an optimal data selection method. We address the following research questions:

\begin{enumerate}
%\item[R1]\label{r1} Can we efficiently increase lexical diversity in large corpus data selection? 
%\item[R1]\label{r1} Can this method still significantly increase the diversity of a corpus?
\item[R1]\label{r1} Can this method select a corpus whose diversity is significantly higher than at random?

\item[R2]\label{r2} Can lexical diversity help construct a morphosyntactically diverse large corpus?

\end{enumerate}
%Other versions of the research questions:

%Can lexical diversity serve as a proxy for morphosyntactic diversity?

%How to promote morphosyntactic diversity in large data selection without calculating it on the fly.

%How to blindly increase morphosyntactic diversity?

%In the process of a large corpus construction,  when morphosyntactic diversity cannot be calculated on the fly, can lexical diversity used as a proxy?

%How to efficiently increase the morphosyntactic diversity of a corpus, without calculating it on the fly? 

%When sampling data from a large corpus with lexical diversity-driven methods, do we obtain a higher morphosyntactic diversity than at random.

This paper is organised as follows. We  introduce formal diversity models and their tractability issues (Sec.~\ref{sec:diversity}), we describe the French source data (Sec.~\ref{sec:data}) and the diversity-driven data selection algorithm used to select an optimally diverse subset of these data (Sec.\ref{sec:data-selection}). Then, we present the experimental diversity-oriented results (Sec.~\ref{sec:evaluation}),  and we discuss conclusion, limitations and future work (Sec.~\ref{sec:conclusions}).

%We present previous work related to treebanking, notably in French, and to diversity quantification (Sec.~\ref{sec:rel_work}). We describe our objectives and constraints (Sec.~\ref{sec:objectives}), we present the source data (Sec.~\ref{sec:cource_data}) and the diversity-driven selection algorithm (Sec.~\ref{sec:data-selection}). We address the parser training (Sec.~\ref{sec:train-data}) and the automatic parsing process of the final corpus (Sec.~\ref{sec:annotation}). We discuss the results in terms of annotation quality and diversity (Sec.~\ref{sec:results}). We finally conclude (Sec.~\ref{sec:conclusions}) and evoke limitations and perspective (Sec.~\ref{sec:limitations}).

  



==> OLD/alg-old.tex <==
\begin{algorithm}
\begin{algorithmic}
%    \State $exhaustivity \gets [5, 3, 1]$
%    \State $voc \gets base$
%    \State $vocbesttext \gets \{\}$
%    \State $besth \gets 0$
%    \State $maxdoc \gets 1000000$
%    \State $maxtok \gets 1000000000$
%    \State $doc \gets 0$
%    \State $tok \gets 0$
%    \State $H \gets H\left(voc\right)$
%    \State $i \gets 0$
%    \State $exh \gets 0$
%    \While{$doc < maxdoc \land tok < maxtok$}
%        \State $\hat{H} = H\left(voc \cup vocthistext\right)$
%        \If{$\hat{H} > H$}
%            \If{$\hat{H} > besth$}
%                \State $besth \gets \hat{H}$
%                \State $vocbesttext \gets vocthistext$
%            \EndIf
%            \State $exh \gets exh + 1$
%            \If{$exh \% exhaustivity[e]$}
%                \State $voc \gets voc \cup vocbesttext$
%                \State $H \gets \hat{H}$
%                \State $exh \gets 0$
%                \State $doc \gets doc + 1$
%                \State $tok \gets tok + \#numtokinthistext$
%            \EndIf
%        \EndIf
%        \State $i \gets i + 1$
%        \If{$i = \#numdocstotal$}
%            \State $e \gets e + 1$
%        \EndIf
%    \EndWhile
%    \Require $I$, a dataset we necessarily include
    \Require $I$, an initial dataset
     \Require $N$, another dataset to select from to enlarge $I$ 
    \Require $E$, a decreasing array of exhaustivity search parameters (positive integers)
    \Require $S$, a maximum size of the resulting dataset $W$
    \Ensure $I$ increased with fragments of $N$ (while maximizing entropy)
    \State $W \gets I$, the working dataset
    %\FOR{\textbf{each} $e \in E$}
    \State $a \gets 0$, counter for which exhaustivity to use
    \While{$a < \left\vert E \right\vert$}
        \State $e \gets E_{a}$
        \State $f \gets 0$, counter for current exhaustivity
        \State $d \gets \emptyset$, document to append
        %\FOR{\textbf{each} $n \in N$}
        \State $b \gets 0$, counter for $N$
        \While{$b < \left\vert N \right \vert$}
            \State $n \gets N_{b}$
            \If{$H\left(W \cup n\right) > H\left(W\right)$}
                \State $f \gets f + 1$
                \If{$H\left(W \cup n\right) > H\left(W \cup d\right)$}
                    \State $d \gets n$
                \EndIf
                \If{$f = e$}
                    \State $W \gets W \cup d$
                    \State $f \gets 0$
                    \State $d \gets \emptyset$
                    \If{$\left\vert W \right\vert > S$}
                        \Return $W$
                    \EndIf
                \EndIf
            \EndIf
            \State $b \gets b + 1$
        %\ENDFOR
        \EndWhile
        \State $a \gets a + 1$
    %\ENDFOR
    \EndWhile
    
    \Return $W$
\end{algorithmic}
\caption{DEPRECATED: Algorithm to heuristically sample data while maximising entropy.\label{alg:heuristic_sample}}
\end{algorithm}
